ALMA observations of fragmentation, sub-structure, and protostars in high-mass starless clump candidates

(Abridged) The initial physical conditions of high-mass stars and protoclusters remain poorly characterized. To this end we present the first targeted ALMA 1.3mm continuum and spectral line survey towards high-mass starless clump candidates, selecting a sample of 12 of the most massive candidates ($400-4000\, M_\odot$) within 5 kpc. The joint 12+7m array maps have a high spatial resolution of $\sim 3000\, \mathrm{au}$ ($\sim 0.8^{\prime\prime}$) and have point source mass-completeness down to $\sim 0.3\, M_\odot$ at $6\sigma$ (or $1\sigma$ column density sensitivity of $1.1\times10^{22}\, \mathrm{cm^{-2}}$). We discover previously undetected signposts of low-luminosity star formation from CO (2-1) and SiO (5-4) bipolar outflows and other signatures towards 11 out of 12 clumps, showing that current MIR/FIR Galactic Plane surveys are incomplete to low- and intermediate-mass protostars ($\lesssim 50\, L_\odot$). We compare a subset of the observed cores with a suite of radiative transfer models of starless cores. We find a high-mass starless core candidate with a model-derived mass consistent with $29^{52}_{15}\, M_\odot$ when integrated over size scales of $2\times10^4\, \mathrm{au}$. Unresolved cores are poorly fit by starless core models, supporting the interpretation that they are protostellar even without detection of outflows. Substantial fragmentation is observed towards 10 out of 12 clumps. We extract sources from the maps using a dendrogram to study the characteristic fragmentation length scale. Nearest neighbor separations when corrected for projection are consistent with being equal to the clump average thermal Jeans length. Our findings support a hierarchical fragmentation process, where the highest density regions are not strongly supported against thermal gravitational fragmentation by turbulence or magnetic fields.

==> commands.tex <==
% General purpose macros
\newcommand{\ee}[1]{\mbox{${} \times 10^{#1}$}}% scientific number format
\newcommand{\eten}[1]{\mbox{$10^{#1}$}}% power of ten
\newcommand{\todo}[1]{\textcolor{red}{#1}}

% Coordinate macros
\newcommand{\uph}{\mbox{$^\mathrm{h}$}}
\newcommand{\upm}{\mbox{$^\mathrm{m}$}}
\newcommand{\ups}{\mbox{$^\mathrm{s}$}}
\newcommand{\degree}{\mbox{$^\circ$}}
\newcommand{\am}{\mbox{\arcmin}}
\newcommand{\as}{\mbox{\arcsec}}

% Unit macros
\newcommand{\cmc}{\ensuremath{
    \mathrm{cm^{-2}}
}}
\newcommand{\cmv}{\ensuremath{
    \mathrm{cm^{-3}}
}}
\newcommand{\kms}{\ensuremath{
    \mathrm{km \ s^{-1}}
}}
\newcommand{\pc}{\ensuremath{
    \mathrm{pc}
}}
\newcommand{\kpc}{\ensuremath{
    \mathrm{kpc}
}}
\newcommand{\um}{\ensuremath{
    \mathrm{\mu m}
}}
\newcommand{\kelvin}{\ensuremath{
    \mathrm{K}
}}
\newcommand{\eupper}{\ensuremath{
    E_\mathrm{u}
}}

% Acronym macros
\newcommand{\akari}{{\it Akari}}
\newcommand{\bgpsfull}{Bolocam Galactic Plane Survey}
\newcommand{\bgpsver}{2.1.0}
\newcommand{\bgps}{BGPS}
\newcommand{\bolocat}{{\tt Bolocat}}
\newcommand{\cutex}{{tt CuTeX}}
\newcommand{\dbscan}{{\tt DBSCAN}}
\newcommand{\ego}{EGO}
\newcommand{\emaf}{EMAF}
\newcommand{\fir}{far-infrared}
\newcommand{\gbtidl}{{\tt GBTIDL}}
\newcommand{\glimpse}{GLIMPSE}
\newcommand{\herschel}{\textit{Herschel}}
\newcommand{\higal}{Hi-GAL}
\newcommand{\hii}{H\textsc{ii}}
\newcommand{\hillf}{\textsc{hill{\footnotesize 5}}}
\newcommand{\hisa}{H\textsc{i}SA}
\newcommand{\hi}{H\textsc{i}}
\newcommand{\irac}{IRAC}
\newcommand{\iras}{\mbox{\it IRAS}}
\newcommand{\iso}{\mbox{\it ISO}}
\newcommand{\mipsgal}{MIPSGAL}
\newcommand{\mir}{mid-infrared}
\newcommand{\mm}{millimeter}
\newcommand{\msx}{\textit{MSX}}
\newcommand{\nirfull}{near-infrared}
\newcommand{\ppv}{PPV}
\newcommand{\sedfull}{spectral energy distribution}
\newcommand{\sed}{SED} % spectral energy distribution
\newcommand{\sfr}{\mbox{$\dot M_{\star}$}} % star-formation rate
\newcommand{\spitzer}{\textit{Spitzer}}
\newcommand{\submm}{submillimeter}
\newcommand{\uchii}{UCH\textsc{ii}}
\newcommand{\wise}{{\it WISE}}

% Physical Variable macros
\newcommand{\alphanir}{\mbox{$\alpha_{NIR}$}} % spectral index 2-20 mic.
\newcommand{\av}{\mbox{$A_V$}} % Visual Extinction
\newcommand{\bperp}{\mbox{$B_{\perp}$}} % Projection of B on plane of sky
\newcommand{\fsmm}{\mbox{$L_{smm}/L_{bol}$}} % submm lum over bol. luminosity
\newcommand{\lbol}{\mbox{$L_\mathrm{bol}$}} % bolometric luminosity
\newcommand{\lsmm}{\mbox{$L_{smm}$}} % luminosity longward of 350 mic.
\newcommand{\lsun}{\mbox{L$_\odot$}}% Lsun
\newcommand{\lsol}{\mbox{L$_\odot$}}% Lsun
\newcommand{\mc}{\mbox{$M_N$}} % column density mass
\newcommand{\mdust}{\mbox{$M_{\rm dust}$}} % dust mass
\newcommand{\meanar}{\mbox{$\langle a/b \rangle$}} % mean aspect ratio
\newcommand{\meanl}{\mbox{$\langle l \rangle$}} % mean size
\newcommand{\mean}[1]{\mbox{$\langle#1\rangle$}} %generic mean for defined qu.
\newcommand{\mn}{\mbox{$M_n$}} % density mass
\newcommand{\msol}{\mbox{M$_\odot$}} % solar mass
\newcommand{\msun}{\mbox{M$_\odot$}} % solar mass
\newcommand{\nbar}{\mbox{$\overline{n}$}}
\newcommand{\nc}{\mbox{$n_c(jk)$}}
\newcommand{\n}{\mbox{$n$}}
\newcommand{\opacity}{\mbox{$\kappa(\nu)$}} % opacity as func. of freq.
\newcommand{\rinf}{\mbox{$r_{inf}$}} % infall radius
\newcommand{\surfdust}{\mbox{$\Sigma_{\rm dust}$}}
\newcommand{\surfhh}{\mbox{$\Sigma_{\rm H_2}$}}
\newcommand{\ta}{{$T_A^*$}} % corrected antenna temperature
\newcommand{\tbol}{\mbox{$T_{bol}$}} % bolometric temperature
\newcommand{\td}{\mbox{$T_\mathrm{d}$}}
\newcommand{\tex}{\mbox{$T_{\rm ex}$}}
\newcommand{\tk}{\mbox{$T_{\rm K}$}}
\newcommand{\tmb}{\mbox{$T_{\rm mb}$}}
\newcommand{\tpk}{\mbox{$T_{\rm pk}$}}
\newcommand{\tr}{\mbox{$T_R$}}
\newcommand{\vlsr}{\mbox{$v_{\rm LSR}$}}

% Molecule name macros
\newcommand{\HII}{\mbox{{\rm H}\,{\scriptsize II}}}
\newcommand{\amm}{\mbox{{\rm NH}$_3$}}
\newcommand{\ccs}{CCS} % CCS
\newcommand{\coooo}{C$^{17}$O}
\newcommand{\cooo}{C$^{18}$O}
\newcommand{\coo}{$^{13}$CO}
\newcommand{\co}{CO} % carbon monoxide
\newcommand{\css}{C$^{34}$S}
\newcommand{\cs}{C$^{32}$S}
\newcommand{\dcop}{DCO$^+$}
\newcommand{\form}{H$_2$CO} % formaldehyde
\newcommand{\hcop}{${\rm HCO}^+$} % HCO+
\newcommand{\htcop}{${\rm H^{13}CO^+}$} % H^13CO+
\newcommand{\hceop}{${\rm HC^{18}O^+}$} % HC^18O+
\newcommand{\hh}{\mbox{${\rm H}_2$}} % H2
\newcommand{\metho}{\mbox{${\rm CH_3OH}$}} % methanol, CH3OH
\newcommand{\sio}{\mbox{${\rm SiO}$}} % silicon-monoxide
\newcommand{\water}{\mbox{${\rm H_2O}$}} % H2O
\newcommand{\nnhp}{\mbox{${\rm N_2H^+}$}} % N2H+
\newcommand{\nndp}{\mbox{${\rm N_2D^+}$}} % N2D+
\newcommand{\hnc}{\mbox{${\rm HNC}$}} % HNC
\newcommand{\dnc}{\mbox{${\rm DNC}$}} % DNC
\newcommand{\hcn}{\mbox{${\rm HCN}$}} % HCN
\newcommand{\htcn}{\mbox{${\rm H^{13}CN}$}} % H^13CN
\newcommand{\hcfn}{\mbox{${\rm HC_5N}$}} % HC5N
\newcommand{\ccchh}{\mbox{${\rm c-C_3H_2}$}} % c-HCCCH


% Molecular transitions macros
\newcommand{\csfifo}{C$^{32}$S $J = 5 \rightarrow 4$}
\newcommand{\cssfifo}{C$^{34}$S $J = 5 \rightarrow 4$}
\newcommand{\cssesi}{C$^{32}$S $J = 7 \rightarrow 6$}


